On correlations between diffuse interstellar bands

One way to better apprehend the problem of diffuse interstellar bands (DIBs) is to search for correlations between the bands in a large sample of spectra towards various lines of sight: a strict correlation may imply that a common carrier is at the origin of the bands, whereas a non-correlation means that different species are involved. We propose this observational test for 10 DIBs collected in up to 62 Galactic lines of sight. Strong DIBs do not strictly correlate, and sometimes the correlation is very poor. Only one example of a strict correlation has been found in our sample between the DIBs at 6614 and 6196 A, that could significate a single carrier for those two bands. The general absence of strict correlations is discussed in the context of molecular carriers for the DIBs.

==> tab1.tex <==
%auto-ignore
HD& 5780&5797&5850&6196&6234&6270&6284&6379&6614\\
2905 && 13.4  (0.3)  &  8.5  (0.4) & 2.3  (0.1)  &  7.0  (0.5) &-&-&-&8.6  (0.3)  & 11.9 (0.5) \\ 	
5394 & & 1.8  (0.2)  &  1.6 (0.3)  & 0.6  (0.2)  & 0.9  (0.4) &-&-&- &6.5  (0.4)  &  1.2 (0.8) \\ 
14489&  & 14.7 (0.4)  &  7.3  (0.3)&  3.0 (0.1)  &  5.0  (0.4)&-&-&- & 5.6  (0.4)  &  9.7  (0.3) \\  
20041 & & 20.2  (0.4)  & 13.0  (0.9) & 4.6  (0.3)  &  9.3  (0.8)&-&-&-&  12.5 (1.3)& 22.4  (1.9) \\  
21291 & & 9.9  (0.2)  &  7.4  (0.4)  &3.1  (0.2) &  4.9  (0.5) &-&-&- & 5.6  (0.2)  &  9.6 (0.5) \\  
21389 & & 19.0  (0.3)  &  8.9  (0.6) & 3.1  (0.2)  &  7.4  (0.5) &-&-&-& 7.6  (0.9)  & 15.0  (0.6) \\  
23180 & & 4.2  (0.2)  &  8.1  (0.6) & 4.6  (0.2) & 3.4  (0.2) &-&-&-&7.0  (0.8)  &  4.5  (0.3) \\	  
22951 & & 5.0  (0.2)  &  4.4  (0.2) & 1.9  (0.1) & 3.8  (0.2) &-&-&-&3.2  (0.3)  &  5.9  (0.3) \\ 	 
24398 & & 5.0  (0.3)  &  7.4  (0.6) & 3.1  (0.4) & 4.1  (0.1) &-&-&-&8.9  (0.8)  &  6.2  (0.2) \\ 	  
24912 & & 9.4  (0.3)  &  5.1  (0.3) & 2.1  (0.1) & 4.6  (0.2) &-&-&-&5.1  (0.7)  &  7.4  (0.5) \\ 	  
37020 & & 2.4  (0.4)  &  1.1  (0.3) & 1.0  (0.2) & 1.3  (0.4) &-&-&-&1.3  (0.4)  &  1.3  (0.6) \\ 
37022 & & 3.0  (0.4)  &  1.0  (0.3)  & 0.7  (0.4) & 1.3  (0.3) &-&-&-&1.1  (0.3  &  1.2  (0.3) \\ 	  
37023 & & 2.8  (0.4)  &  1.4  (0.3) & 1.0  (0.2) & 1.4  (0.2) &-&-&-&1.4  (0.2)  &  1.3  (0.1) \\ 
34078 && 8.1  (0.4)  &  5.6  (0.3) & 2.3  (0.3) & 3.7  (0.3) &-&-&-&2.2  (0.3)  &  4.8  (0.5) \\ 
41117 & & 16.0  (0.2)  & 14.0  (0.6)  &  5.6  (0.3) & 8.3  (0.3) &-&-&-&16.3 (1.7)  & 15.6  (0.7) \\  
42087 &&  11.7  (0.3)  & 10.6  (0.8)  &  5.6  (0.3) & 6.5  (0.4)  &-&-&-& 7.6  (0.3)  & 11.5  (0.9) \\  
43384 && 20.7  (0.5)  & 14.1  (0.9)  &  5.0  (0.2)  & 11.2  (1.1) &-&-&-&  12.1  (1.5)  & 19.1 (1.2) \\  
41335 & & 1.4  (0.1)  &  1.3  (0.1)  & 0.8  (0.1)  &  2.1  (0.3)  &-&-&-& 1.3  (0.2) & 3.2  (0.3) \\
89353 &&  1.7  (0.3)  &  1.3  (0.1)  &  1.1  (0.2)   &  1.0  (0.2)  &0.5 (0.2)&1.3 (0.1) &1.2 (0.2)  & 1.1  (0.2)   &  0.7  (0.3) \\
141637 & & 4.2  (0.1)   &  1.2  (0.1)   &  1.1  (0.3)   &  1.8  (0.1) &0.7 (0.1)&1.9 (0.2)&3.7 (0.4) & 1.6  (0.1)  &  2.1  (0.3) \\ 
142114 && 3.5  (0.2)   &  1.2  (0.1)   & 0.7  (0.1)   &  1.7  (0.1)  &0.4 (0.1)&1.4 (0.1) &3.1 (0.5)  & 1.5  (0.1)   &  1.4  (0.1) \\
143275 & & 9.8  (0.3)   &  2.0  (0.1)  & 1.0  (0.1)   &  1.9  (0.2) &0.5 (0.1) &1.2 (0.1) &3.0 (0.3)  & 1.6 (0.1)   &  1.5  (0.1) \\
144470 & & 0.9  (0.1)  &  3.2  (0.2) & 1.3  (0.2)  &  3.9  (0.3)  &1.3 (0.1) &2.1(0.3)&4.6 (0.2)& 4.2  (0.1)  &  6.4  (0.3) \\
145502 &5.7(0.6) & 8.5  (0.2)  &  3.8  (0.2)  &  1.5  (0.1)  &  3.2  (0.1)  &1.3 (0.2) &1.1 (0.3)&5.7 (0.2) & 4.6  (0.2)  &  6.0  (0.3) \\  	   
147165 & & 12.0  (0.5)  &  3.6  (0.1)  &  1.6  (0.3)  &  3.7  (0.1) &1.6 (0.2) &1.3 (0.3)&5.1 (0.2) & 4.0  (0.2)  &  5.7  (0.3)\\  
147933 & & 10.1  (0.2)  &  6.7  (0.1)  &  2.9  (0.5)  &  3.4  (0.3) &1.2 (0.2) &1.2 (0.2)&3.6 (0.4) & 4.0  (0.1)  &  5.2  (0.3) \\ 
148184 & & 5.5  (0.3)  &  5.3  (0.2)  &  3.4  (0.2)  &  2.4  (0.2) &1.2 (0.2) &1.1 (0.2)&2.8 (0.3) & 4.2 (0.2)  &  4.2  (0.5) \\ 
149757 &3.7 (0.4) & 3.7  (0.1)  &  4.1  (0.1)  &  1.9  (0.1)  &  2.5  (0.1) &1.0 (0.2) &1.1 (0.1)&2.0 (0.1) & 3.5 (0.2)  &  3.4  (0.1) \\  	   	
154445 &4.7(0.5) & 9.7  (0.3)  &  7.9  (0.5)  &  2.8  (0.2)  &  5.7  (0.5) &1.8 (0.2) &3.1 (0.3)&4.1 (0.3)  & 7.8  (0.2)  & 11.8  (0.9) \\ 	   	
164402 & & 7.2  (0.4)  &  4.4  (0.2)  &  2.6  (0.3)  &  4.0  (0.4) &1.2 (0.1)&1.6 (0.1)&3.0 (0.1) & 3.8  (0.1)  &  4.0  (0.5) \\ 
166937 & & 12.3  (0.5)  &  9.2  (0.6)  &  3.8  (0.5)  &  5.7  (0.5) &1.7 (0.2)&3.3 (0.2)&8.1 (0.2)& 8.3 (0.2)  &  9.4  (0.4)\\ 
179406 & & 8.2  (0.3)  &  8.4  (0.6)  &  4.1  (0.2)  &  4.8  (0.1) &1.3 (0.4)&2.8 (0.2)&2.7 (0.2) & 9.7  (0.4)  &  9.0  (0.4) \\  
184915 &5.9 (0.6) & 7.6  (0.2)  &  3.1  (0.2)  &  1.1  (0.1)  &  4.4  (0.1)&0.8 (0.2)&2.6 (0.3)&3.6 (0.3) & 3.8  (0.2)  &  6.9  (0.6) \\	   
198478 &6.7(0.7) & 14.2  (0.9)  &  9.0  (0.6)  &  3.6  (0.2)  &  7.0  (0.2)&2.1 (0.1)&3.9 (0.4)&3.9 (0.5) & 9.5  (0.1)  & 12.4  (0.6) \\	  
199579 & & 5.4  (0.3)  &  5.5  (0.5) & 2.6  (0.2  &  3.2  (0.2)&2.0 (0.3)&1.2 (0.1)&3.68 (0.4)& 2.9  (0.3)  &  4.8  (0.6) \\
203064 & & 7.7  (0.3)  &  5.5  (0.5) & 2.4  (0.4)  &  3.7  (0.2)&1.6 (0.2)&2.0 (0.2)&6.0 (0.6) & 2.9  (0.2)  &  6.7  (0.6) \\
206165 &5.9 (0.6) & 9.5  (0.9)  &  8.9  (0.2) & 3.8  (0.4)  &  5.6  (0.2)&1.4 (0.1)&2.9 (0.3)&6.8 (0.7)& 8.4  (0.1)  & 10.5  (0.5) \\
206267 & & 10.3  (0.2)  &  9.9  (0.4) & 4.5  (0.3)  &  6.2  (0.5)&2.1 (0.3)&3.1 (0.3)&7.1 (0.7) & 6.2 (0.3)  & 11.3  (0.5) \\
207260 &5.9 (0.6) & 14.8  (0.4)  & 11.0  (0.9) & 4.0  (0.2)  &  7.0  (0.7)&1.8 (0.2)&4.9 (0.5)&9.3 (0.9) & 11.5 (0.2)  & 13.6  (0.8) \\  
208501 &5.2 (0.5) & 10.9  (0.3)  & 11.0  (0.9) & 3.8  (0.3)  &  6.5  (0.4)&2.0 (0.3)&3.5 (0.4)&6.7 (0.8) & 8.5 (0.3)  & 11.8  (0.5) \\	   
210839 & & 11.4  (0.4)  &  9.6  (0.6) & 3.1  (0.2)  &  7.4  (0.4) &1.9 (0.1)&5.2 (0.5)&7.5 (0.8)& 8.4 (0.1)  & 14.3  (0.4) \\
209975 & & 11.8  (0.3)  &  8.7  (0.2) & 3.3  (0.2)  &  6.2  (0.2)&2.0 (0.1)&3.8 (0.4)&8.0 (0.8) & 7.2  (0.1)  & 11.6  (0.7)\\
54662  && 9.5  (0.3)  &  6.3  (0.3)  &  2.8  (0.3)  &  4.5  (0.3)&1.6 (0.5)&3.3 (0.4)&8.8 (0.9) & 5.2  (0.5)  &  8.8  (0.6) \\
207198 & & 11.1  (0.2)  & 16.0  (1.2)  &  8.5  (0.3)  &  6.7  (0.2)&2.7 (0.1)&3.9 (0.4)&7.9 (0.8)& 11.8  (0.3)& 12.6  (0.9) \\
209481 & & 8.5  (0.4)  &  6.8  (0.8)  &  2.9  (0.4)  &  5.1  (0.1) &1.5 (0.4)&3.5 (0.4)&6.8 (0.7)& 11.8 (0.4)& 9.6  (0.7)\\
24534  &2.5 (0.3)& 4.6  (0.2)  &  7.5  (0.4) &  4.4  (0.6)  &  3.8  (0.2) &1.8 (0.3) &2.0 (0.2)&3.5 (0.5)&  7.4  (0.3) & 5.8  (0.5) \\	 
212076 & & 1.7  (0.4) & 1.6  (0.2) & 0.8  (0.2) &  1.3  (0.1) &0.8 (0.2)&2.0 (0.2)&2.0 (0.2)& 1.5  (0.2) & 1.3  (0.2)\\
218376 & & 5.9  (0.3) & 4.8  (0.2) & 1.8  (0.2) & 3.6  (0.2) &1.1 (0.2)&2.9 (0.3)&5.1 (0.5) & 5.5  (0.3)&  6.5  (0.4)\\
223128 & & 6.4  (0.4)& 6.3  (0.3) & 2.4  (0.4) & 3.8  (0.2) &1.1 (0.2)&2.8 (0.3)&4.8 (0.5)& 5.5  (0.2)&  6.6  (0.3)\\
47129  && 8.2  (0.4)& 5.1  (0.3) & 1.8  (0.5)& 4.2  (0.2) &0.6(0.2)&5.0(0.5)&6.7(0.7) & 5.1  (0.2) &  8.1  (0.5)\\
47099  && 8.8  (0.4) & 0.1  (0.1) & 5.4  (0.3) & 3.9  (0.2)  &-&-&-&3.4  (0.5) & 8.7  (0.4) \\
37061 & & 6.8  (2.0) & 1.6  (0.1)  & 0.9  (0.2) & 1.6  (0.4)  &-&-&-& 1.8 (0.5) & 1.6  (0.1)\\
37042 & & 1.9  (0.1)  & 0.9  (0.2)  & 0.7  (0.1)  & 0.9  (0.2)  &-&-&-&1.8  (0.1) & 1.8  (0.2)\\
47240  && 11.2  (0.9) & 8.4  (0.6) & 3.4  (0.3) & 5.7  (0.6)  &-&-&- &7.4  (0.7) &10.9  (0.9)\\
224572 & & 3.6  (0.2) & 2.8  (0.2) & 1.5  (0.3) & 2.2  (0.2)  &-&-&-&1.7  (0.2) & 4.0  (0.3) \\
213420 & & 4.1  (0.1)   & 2.6  (0.1)   & 1.6  (0.1)   & 1.9  (0.2)  &-&-&-&1.7  (0.1)   & 3.5  (0.2)  \\
216200 & & 4.6  (0.5)   & 5.3  (0.5)   & 2.6  (0.2)   & 2.2  (0.1)    &-&-&-&2.7  (0.1)   & 4.3  (0.1)  \\
144217 &7.7 (0.8)  & 8.4  (0.2)   & 2.2  (0.1)    & 0.7  (0.2)   & 3.0  (0.2) &-&-&-& 2.5  (0.3)  &  5.3  (0.6)  \\	
142184 & & 3.8  (0.1)   & 2.2  (0.1)   & 1.1  (0.3)   & 1.9  (0.4)   &-&-&-&2.2  (0.1)   & 2.3  (0.1)  \\
24760  && 3.5  (0.5)  & 1.8  (0.1)    & 0.8  (0.1)  &  2.1  (0.3)    &-&-&-&1.3  (0.2)   & 3.2  (0.3) \\
13267  && 11.6  (0.2)   & 6.5  (0.3)  &  2.3  (0.2)   & 4.9  (0.2)    &-&-&-&6.5  (0.6)   &10.6  (0.8) \\
183143 &15.4(0.9)  & 34.1  (0.9)   &20.3  (1.5)  & 7.0  (0.5)  & 14.6  (0.9) &-&-&-& 15.7 (1.5)  & 29.2  (0.9)  \\


==> tab2.tex <==
%auto-ignore
HD&Sp T & E(B-V)& m$_v$& V$sin$i&HD&Sp T & E(B-V)& m$_v$& V$sin$i\\
&&&&&144217&B0.5 V&0.17&2.62 &130\\
2905 & B1 I  & 0.33& 4.16   & 62&144470&B1 V&0.19&3.96&142\\
5394 & B0 IV  & 0.10  & 2.47   & 300   &145502   & B3 V& 0.25&4.01&199\\
8065&A0 I&0.39&6.46&--&147084&A4 III&0.96&4.55&15\\
10516 & B2 V  & 0.17  & 4.07   & 450   &147165& B2 III + O9.5 V& 0.36& 2.89& 53 \\
12953&A1 I&0.62&6.28&30&147933&B2 IV&0.44&5.02&303  \\
13267 & B5 I  & 0.41  & 6.36   & 53   & 148184&B2 IV&0.48&4.42&134  \\
14489 & A2 I  & 0.40  & 5.17  & 25   & 149757   &    O9.5 V   &     0.29    &    2.56 & 379 \\
20041 & A0 I&0.73 &5.79  & --  & 154445   &    B1   V   &     0.39    &    5.64 &174 \\
21291 &B9 I & 0.42 &4.21  & 29 & 163472   &    B2 IV-V  &     0.30    &    5.82     &  120 \\
 21389 &    A0 Iae   &    0.56 & 4.54 &6 & 164284 & B2 Ve &   0.18&  4.64  &  221  \\
 22951 & B0 V & 0.23  &  4.97  &  51&164353   & B5  Ib  &  0.23 &3.97 &  22\\
 23180 & B1 III&0.26&3.82 & 85 & 164402&B0 I&0.22&5.77&100 \\
 24398 &B1 Ib&0.31 & 2.85 & 59 &166182&B2 IV&0.04&4.36&-\\
 24534 & O9.5pe& 0.56 &6.10 & 150  &166937&B8 I&0.34&3.86&54 \\
 24760 &B0.5 V + A2 V &0.06 & 2.89&153 &170740&B2 V&0.45&5.72&-\\
 24912 & O7.5 III & 0.29 & 4.02 & 216 & 179406  &  B3 V &0.31& 5.34&187 \\
 25204&B3 V + A4 IV&0.30&3.47&75&183143 & B7 Iae & 1.28& 6.86& 59 \\
 34078   & O9.5 V & 0.50 & 8.00  & 5 & 184915  & B0.5 III & 0.22& 4.95  &259 \\
 37020   & B3 V & 0.37 & 6.36 & 112& 193237& B2 pe & 0.61& 4.81 &75  \\
 37022   & B8 III & 0.96& 8.31 &127 &198478&B3 Iae&0.54&4.84 &35  \\
 37023   & O9.5 Iae &0.26 & 4.29 & 109&199478&B8 I&1.00&5.67&-\\
 37042&B1 V&0.32&6.39&-&199579&O6 Ve&0.34& 5.96 &  170 \\
 37061&B1 V&0.50&6.82&-&202850&B9 Iab&0.13& 4.23  &  28 \\
 40111&B0.5 II&0.28&4.76&130&202904&B2 V&0.10&4.43&261 \\
 41117 &B2 Ia & 0.44&4.63& 36&203064 &  O8 e & 0.28    &    5.00     &  328\\
 41335 &B2 V &0.15 &5.21 &419 & 206165   &    B2 Ib &0.46&4.73 &36 \\
 42087 &  B2.5 I &0.35 &5.75 &37& 206267   &    O6   f   &     0.50    &    5.62     &  154\\
 43384& B3 I&0.58 &  6.25  &51&207198&O9 II &0.56&5.95& 76  \\
 45725& B3 V  &0.08 &4.60  &346    &207260   &    A2  Ia   &     0.50    &    4.29 &33 \\
 48099& O6 e  & 0.34 &6.37 & -- &208501   &    B8  Ib   &     0.75    &    5.80     &  53 \\
 47129& O8 V&0.33 &6.06  &80  &209481&O9 V&0.34&5.56 &130 \\
 47240&B1 I &0.33&6.15 & 126&209975&O9 I&0.33&5.11 &33 \\
 54662&O7 III& 0.27&6.21 &91&210839 &O6 If& 0.46&5.04 &  285 \\
 89353&B9.5 I&  0.24 &5.34 &-- & 212076&B2 IV&0.08&5.01&134  \\
141637 & B3 V  & 0.13 &4.64 &300 &213420&B2 IV&0.16&5.95 & --\\
142096&B3 V&0.20&5.02&207&216200&B3 IV& 0.25 & 5.92& 225 \\
142114 &B2.5 V&0.12&4.59&308&218376&B0.5 IV  & 0.21 &4.85 &  50   \\
142184 &B2.5 V&0.15&5.42&349&223128&B2 IV&0.16&5.95&-- \\
143275 &B0.5 IV&0.12&2.32&181&224572&B1 V &0.16&4.88&189  \\
\hline 

